Building a Winning Self-Driving Car in Six Months

The SAE AutoDrive Challenge is a three-year competition to develop a Level 4 autonomous vehicle by 2020. The first set of challenges were held in April of 2018 in Yuma, Arizona. Our team (aUToronto/Zeus) placed first. In this paper, we describe our complete system architecture and specialized algorithms that enabled us to win. We show that it is possible to develop a vehicle with basic autonomy features in just six months relying on simple, robust algorithms. We do not make use of a prior map. Instead, we have developed a multi-sensor visual localization solution. All of our algorithms run in real-time using CPUs only. We also highlight the closed-loop performance of our system in detail in several experiments.

==> sections/sensor_fusion.tex <==
\section{Sensor Fusion}

Several components in our system rely on fusion of sensor data. Stop signs are detected in camera images while we use the LIDAR to estimate distance to stop signs. Obstacle detection combines lane detection in images with obstacle detection from LIDAR point clouds. Finally, we combine lane detection results from both camera and LIDAR. In order to fuse camera and LIDAR data we need an accurate extrinsic calibration between the sensors. We made use of two camera to LIDAR calibration libraries \cite{Unnikrishnan2005, Geiger2012}. Unnikrishnan et al. \cite{Unnikrishnan2005} use one checkered calibration target that is moved to around 20 different poses in the camera's field of view. The target is automatically detected in the image, while we manually mark it in the point cloud. Geiger et al. \cite{Geiger2012} use several calibration targets in one frame. The calibration targets are automatically detected in both the image and point cloud. The second approach reduces the number of frames we need to collect, but requires several calibration targets. Moreover, the targets need to be placed at different angles covering all of the camera field of view, which is more challenging to set up.     

==> sections/software_arch.tex <==
\begin{figure}[ht]
    \includegraphics[width=\columnwidth]{figs/SoftwareArchitecture.png}
    \centering
    \caption{Zeus' software architecture. M: Monocular camera, L: 3D LIDAR, G: GPS/IMU, S: Stereo camera. The Trajectory Planner and Finite State Machine (FSM) determines our current state (lane-keeping | stopping | lane-changing) and outputs a sequence of waypoints.}
    \label{fig:software_arch}
\end{figure}

\section{Software Architecture}

Zeus' software architecture is shown in Figure~\ref{fig:software_arch}. Our perception nodes include Stop-Sign/Line Detection, Lane Detection, Pose Estimation, and Occupancy Mapping. The Trajectory Planner and Finite State Machine (FSM) determines our current state (lane-keeping | stopping | lane-changing) and outputs a sequence of waypoints. These are then consumed by the Path Tracking Controller node, which in turn provides torque and acceleration commands to our vehicle interface.
